Trident: Efficient 4PC Framework for Privacy Preserving Machine Learning

Machine learning has started to be deployed in fields such as healthcare and finance, which propelled the need for and growth of privacy-preserving machine learning (PPML). We propose an actively secure four-party protocol (4PC), and a framework for PPML, showcasing its applications on four of the most widely-known machine learning algorithms -- Linear Regression, Logistic Regression, Neural Networks, and Convolutional Neural Networks. Our 4PC protocol tolerating at most one malicious corruption is practically efficient as compared to the existing works. We use the protocol to build an efficient mixed-world framework (Trident) to switch between the Arithmetic, Boolean, and Garbled worlds. Our framework operates in the offline-online paradigm over rings and is instantiated in an outsourced setting for machine learning. Also, we propose conversions especially relevant to privacy-preserving machine learning. The highlights of our framework include using a minimal number of expensive circuits overall as compared to ABY3. This can be seen in our technique for truncation, which does not affect the online cost of multiplication and removes the need for any circuits in the offline phase. Our B2A conversion has an improvement of $\mathbf{7} \times$ in rounds and $\mathbf{18} \times$ in the communication complexity. The practicality of our framework is argued through improvements in the benchmarking of the aforementioned algorithms when compared with ABY3. All the protocols are implemented over a 64-bit ring in both LAN and WAN settings. Our improvements go up to $\mathbf{187} \times$ for the training phase and $\mathbf{158} \times$ for the prediction phase when observed over LAN and WAN.

==> Main_SecModel.tex <==
\subsection{Architecture}
\subsection{Security Defination}

==> Main_Semantics.tex <==
%-----
%\subsection{Types of Secret Sharing} 
%\label{sec:sharetypes}
%-----
In this section, we explain three variants of secret sharing that are used in this work. The sharing works over both arithmetic ($\Z{\ell}$) and boolean ($\Z{1}$) rings.
%---
\paragraph{\bf $\sqd$-sharing}
%---
A value $\val$ is said to be $\sqd$-shared among parties $\ESet$, if the parties $P_1, P_2$ and $P_3$ respectively holds the values $\val_1, \val_2$ and $\val_3$ such that $\val = \val_1 + \val_2 + \val_3$. We use $\sqd_{P_i}$ to denote the $\sqd$-share of  party $P_i$ for $i \in \EInSet$.
%---
\paragraph{\bf $\sgrd$-sharing}
%---
A value $\val$ is said to be $\sgrd$-shared among parties $\ESet$, if the parties $P_1, P_2$ and $P_3$ respectively holds values $(\val_1, \val_2), (\val_2, \val_3)$ and $(\val_3, \val_1)$ such that $\val = \val_1 + \val_2 + \val_3$. We denote $\sgrd$-share of the parties as follows:
%{\small
	\begin{center}
		$\sgr{\val}_{P_1} = (\val_1, \val_2),~\sgr{\val}_{P_2} = (\val_2, \val_3),~\sgr{\val}_{P_3} = (\val_3, \val_1)$
	\end{center}
%}
%---
\paragraph{\bf $\shrd$-sharing}
%---
A value $\val$ is said to be $\shrd$-shared among parties $\PSet$, if 
\begin{myitemize}
	%---
	\item[--] there exists values $\Pad{\val}, \Mask{\val}$ such that $\Mask{\val} = \val + \Pad{\val}$.
	%---
	\item[--] parties $\ESet$ know the value $\Mask{\val}$ in clear, while the value $\Pad{\val}$ is $\sgrd$-shared among them. i.e., $\sgr{\Pad{\val}}_{P_1} = (\PadA{\val}, \PadB{\val}), \sgr{\Pad{\val}}_{P_2} = (\PadB{\val}, \PadC{\val}),  \sgr{\Pad{\val}}_{P_3} = (\PadC{\val}, \PadA{\val})$.
	%---
	\item[--] party $P_0$ knows $\PadA{\val}, \PadB{\val}$ and $\PadC{\val}$ in clear.
	%--- 
\end{myitemize}
%
We denote $\shrd$-share of the parties as follows:
%{\small
	\begin{align*}
	\shr{\val}_{P_0} &= (\PadA{\val}, \PadB{\val}, \PadC{\val}) \\
	\shr{\val}_{P_1} &= (\Mask{\val}, \PadA{\val}, \PadB{\val}) \\
	\shr{\val}_{P_2} &= (\Mask{\val}, \PadB{\val}, \PadC{\val}) \\
	\shr{\val}_{P_3} &= (\Mask{\val}, \PadC{\val}, \PadA{\val}) 
	\end{align*}
%}
%
We use $\shr{\val} = (\Mask{\val}, \sgr{\Pad{\val}})$ to denote the $\shrd$-share of $\val$. 
%------
\paragraph{Linearity of the secret sharing schemes}
%------
Given the $\sqd$-sharing of $\wx, \wy$ and public constants $c_1, c_2$, parties can locally compute $\sqr{c_1 \wx + c_2 \wy}$. To see this,
\begin{align*}
\sqr{c_1 \wx + c_2 \wy} &= (c_1 \wx_1 + c_2 \wy_1, c_1 \wx_2 + c_2 \wy_2, c_1 \wx_3 + c_2 \wy_3)\\
&= c_1 \sqr{\wx} + c_2 \sqr{\wy}
\end{align*}
It is easy to see that the linearity trivially extends to $\sgrd$-sharing as well. That is $\sgr{c_1 \wx + c_2 \wy} = c_1 \sgr{\wx} + c_2 \sgr{\wy}$. Similarly, given the $\shrd$-sharing of $\wx, \wy$ and public constants $c_1, c_2$, parties can locally compute $\shr{c_1 \wx + c_2 \wy}$.
\begin{align*}
	\shr{c_1 \wx + c_2 \wy} &= (c_1 \Mask{\wx} + c_2 \Mask{\wy}, c_1 \sgr{\Pad{\wx}} + c_2 \sgr{\Pad{\wy}})\\
							&= c_1 \shr{\wx} + c_2 \shr{\wy}
\end{align*}
The linearity property enables parties to perform the operations of addition as well as multiplication with a public constant locally.

==> figures/abstraction.tex <==
\begin{tikzpicture}

\draw [thick] (-2,2) rectangle (1,0);
\node (A) at (-0.5, 1) {$g = e ((uv)+c)$};
\node (A1) at (-3, 1.8) {$u$};  \node (A2) at (-1.89, 1.8) {}; \draw [-stealth , thick] (A1) -- (A2);
\node (B1) at (-3, 1.3) {$v$};   \node (B2) at (-1.89, 1.3) {}; \draw [-stealth , thick] (B1) -- (B2);
\node (C1) at (-3, 0.8) {$c$};         \node (C2) at (-1.89, 0.8) {}; \draw [-stealth , thick] (C1) -- (C2);
\node (D1) at (-3, 0.3) {$e$};        \node (D2) at (-1.89, 0.3) {}; \draw [-stealth , thick] (D1) -- (D2);
\node (E1) at (0.87,1) {};         \node (E2) at (2, 1) {$g$};       \draw [-stealth , thick] (E1) -- (E2);
\end{tikzpicture}

==> figures/aby3_bench.tex <==
\begin{tikzpicture}

\node(Y) [circle, thick, draw, inner sep=0pt, minimum width=2cm,font=\bfseries]   at (0,6.7) {\Large Y};
\node (A) [circle, thick, draw, inner sep=0pt, minimum width=2cm,font=\bfseries]  at (-4.1, 0) {\Large A};
\node (B) [circle, thick, draw, inner sep=0pt, minimum width=2cm,font=\bfseries]  at (+4.1, 0) {\Large B};

\path [->, thick] [bend left = 25] (Y) edge (B);
\path [->, thick] (B) edge (Y);

\path [->, thick] [bend left = 25] (A) edge (Y);
\path [->, thick] (Y) edge (A);


\path [<->, thick] [bend right =25] (A) edge (B);


\node at (0, 9.3) {
  \begin{tabular}{|c||cc|cc|}
  \hline
  \multicolumn{5}{|c|}{Yao Sharing} \\
  \hline
  Op & \multicolumn{2}{|c|}{Offline Time} & \multicolumn{2}{|c|}{Online Time}\\  \cline{2-5}
        & local & cloud & local & cloud\\
  \hline \hline
  Share & 1.7 & 4.6         & 24.3  & 154857.6\\
  Rec    & 0    & 0            & 8.8    & 86315.5\\
  XOR   & 0    & 0            & 0      & 0\\
  AND  & 6.3 & 85473.6  & 9.1    & 11.2\\
  \hline
  \end{tabular}
 };
 

\node at (-4.1, -3) {
  \begin{tabular}{|c||cc|cc|}
  \hline
  \multicolumn{5}{|c|}{Arithmetic Sharing} \\
  \hline
  Op & \multicolumn{2}{|c|}{Offline Time} & \multicolumn{2}{|c|}{Online Time}\\  \cline{2-5}
       & local & cloud & local & cloud\\
  \hline \hline
  Share   & 13.2  & 68705.8   &12.9   & 72550.2\\
  Rec      & 0       & 0              & 9.6    & 70192.0\\
  ADD    & 0       & 0              &0       &0\\
  MUL    & 13.9  & 73075.8   &12.1   &283571.4\\
  \hline
  \end{tabular}
 };
 
 \node at (4.1, -3) {
  \begin{tabular}{|c||cc|cc|}
  \hline
  \multicolumn{5}{|c|}{Boolean Sharing} \\
  \hline
   Op & \multicolumn{2}{|c|}{Offline Time} & \multicolumn{2}{|c|}{Online Time}\\  \cline{2-5}
        & local & cloud  & local & cloud\\
  \hline \hline
  Share  & 14.5  & 69131.3     & 13.1   & 69064.7\\
  Rec     & 0       & 0                & 10.6   & 72709.9\\
  XOR    & 0       & 0               & 0        & 0\\
  AND    & 14.2  & 68728.7    & 13.8   & 264700.1\\
  \hline
  \end{tabular}
 };
 
  \node at (-5.4, 4.8) {
	\begin{tabular}{|c|cc|}
	\hline
	\multicolumn{3}{|c|}{A2Y} \\
	\hline
	 & local & cloud \\
	\hline \hline
	SetUp  & 22.5 & 164276.5\\
	Online & 26.3 & 168427.2\\
	\hline
	\end{tabular}
 };
 
  \node at (5.4, 4.8) {
	\begin{tabular}{|c|cc|}
	\hline
	\multicolumn{3}{|c|}{Y2B} \\
	\hline
	 & local & cloud \\
	\hline \hline
	SetUp  & 0      & 0\\
	Online & 10.9 & 69339.4\\
	\hline
	\end{tabular}
 };

 
 \node at (0, 0.15) {
	\begin{tabular}{|c|cc|}
	\hline
	\multicolumn{3}{|c|}{B2Y} \\
	\hline
	 & local & cloud \\
	\hline \hline
	SetUp  & 22.7  & 158584.8\\
	Online & 21.9  & 166733.8\\
	\hline
	\end{tabular}
 };
 
  \node at (0,2.1) {
	\begin{tabular}{|c|cc|}
	\hline
	\multicolumn{3}{|c|}{Y2A} \\
	\hline
	 & local & cloud \\
	\hline \hline
	SetUp  & 22.8 & 164354.5\\
	Online & 10.1 & 74499.8\\
	\hline
	\end{tabular}
 };

\end{tikzpicture}

==> figures/aby3_offline.tex.preview.tex <==
%& C:\Users\ajith\AppData\Roaming\TikzEdt\TikzEdt\023~1.0\TEMP_H~1
\begin{document}
\begin{tikzpicture}

\node (Y) [circle, thick, draw, inner sep=0pt, minimum width=2cm]   at (0,7) {Y};
\node (A) [circle, thick, draw, inner sep=0pt, minimum width=2cm]  at (-5, 0) {A};
\node (B) [circle, thick, draw, inner sep=0pt, minimum width=2cm]  at (+5, 0) {B};

\path [->, thick] [bend left = 25] (Y) edge (B);
\path [->, thick] (B) edge (Y);

\path [->, thick] [bend left = 25] (A) edge (Y);
\path [->, thick] (Y) edge (A);


\path [<->, thick] [bend right =25] (A) edge (B);


\node at (0, 9.5) {
  \begin{tabular}{|c||cc|}
  \hline
  \multicolumn{3}{|c|}{Yao Sharing} \\
  \hline
  Op & local & cloud \\
  \hline \hline
  Share & 0 & 0\\
  XOR & 0 & 0\\
  AND & 0 & 0\\
  \hline
  \end{tabular}
 };

\node at (-8.5, 0) {
  \begin{tabular}{|c||cc|}
  \hline
  \multicolumn{3}{|c|}{Arithmetic Sharing} \\
  \hline
  Op & local & cloud \\
  \hline \hline
  Share & 0 & 0\\
  ADD & 0 & 0\\
  MUL & 0 & 0\\
  \hline
  \end{tabular}
 };
 
 \node at (8.5, 0) {
  \begin{tabular}{|c||cc|}
  \hline
  \multicolumn{3}{|c|}{Boolean Sharing} \\
  \hline
  Op & local & cloud \\
  \hline \hline
  Share & 0 & 0\\
  XOR & 0 & 0\\
  AND & 0 & 0\\
  \hline
  \end{tabular}
 };
 
  \node at (-6, 4) {
	\begin{tabular}{|cc|}
	\hline
	\multicolumn{2}{|c|}{A2Y} \\
	\hline
	local & cloud \\
	\hline \hline
	0 & 0\\
	\hline
	\end{tabular}
 };
 
  \node at (6, 4) {
	\begin{tabular}{|cc|}
	\hline
	\multicolumn{2}{|c|}{Y2B} \\
	\hline
	local & cloud \\
	\hline \hline
	0 & 0\\
	\hline
	\end{tabular}
 };

 
 \node at (2, 1.5) {
	\begin{tabular}{|cc|}
	\hline
	\multicolumn{2}{|c|}{B2Y} \\
	\hline
	local & cloud \\
	\hline \hline
	0 & 0\\
	\hline
	\end{tabular}
 };
 
  \node at (-2,1.5) {
	\begin{tabular}{|cc|}
	\hline
	\multicolumn{2}{|c|}{Y2A} \\
	\hline
	local & cloud \\
	\hline \hline
	0 & 0\\
	\hline
	\end{tabular}
 };


\usetikzlibrary{calc}
\pgftransformreset
\node[inner sep=0pt,outer sep=0pt,minimum size=0pt,line width=0pt,text width=0pt,text height=0pt] at (current bounding box) {};
%add border to avoid cropping by pdflibnet
\foreach \border in {0.1}
  \useasboundingbox (current bounding box.south west)+(-\border,-\border) rectangle (current bounding box.north east)+(\border,\border);
\newwrite\metadatafile
\immediate\openout\metadatafile=\jobname_BB.txt
\path
  let
    \p1=(current bounding box.south west),
    \p2=(current bounding box.north east)
  in
  node[inner sep=0pt,outer sep=0pt,minimum size=0pt,line width=0pt,text width=0pt,text height=0pt,draw=white] at (current bounding box) {
\immediate\write\metadatafile{\p1,\p2}
};
\immediate\closeout\metadatafile
\end{tikzpicture}

\end{document}
}

}

}
}
}
}

}


\end{document}


\end{document}


\end{document}


==> symbols.tex <==
%\input{symbols/symbols_main}

%-----------------------------
%Math Symbols
%-----------------------------
\input{symbols/symbols_maths}

%-----------------------------
%Environments Symbols
%-----------------------------
\input{symbols/symbols_env}

%-----------------------------
%Circuit Symbols
%-----------------------------
\input{symbols/symbols_ckt}

%-----------------------------
%MPC Symbols
%-----------------------------
\input{symbols/symbols_mpc}

%-----------------------------
%4PC Symbols
%-----------------------------
\input{symbols/symbols_4pc}

%-----------------------------
%Garbled Symbols
%-----------------------------
\input{symbols/symbols_garbled}

%-----------------------------
%Conversions Symbols
%-----------------------------
\input{symbols/symbols_conv}

%-----------------------------
%ML Symbols
%-----------------------------
\input{symbols/symbols_ml}

%-----------------------------
%Temp Symbols
%-----------------------------
%\input{symbols/symbols_temp}

==> symbols/symbols_3pc.tex <==
%--------------------------------------------------------------
%ThreePC Variables and Notations
%--------------------------------------------------------------

\newcommand{\sq}{\ensuremath{[\cdot]}}
\newcommand{\sqr}[1]{[ #1 ]}
\newcommand{\grp}[1]{ \langle #1 \rangle}

\newcommand{\mask}[1]{\ensuremath{\mathsf{m}_{#1}}}
\newcommand{\mstar}[1]{\ensuremath{\mathsf{m}_{#1}^{\star}}}

\newcommand{\masked}[1]{\ensuremath{\mathsf{m}_{#1}}}
\newcommand{\starmasked}[1]{\ensuremath{\mathsf{m}_{#1}^{\star}}}

\newcommand{\Value}{\ensuremath{\mathsf{Val}}}
\newcommand{\val}[1]{\ensuremath{{#1}_{\mathsf{v}}}}

%--------------------------------------------------------------
%ThreePC Protocols and SubProtocols
%--------------------------------------------------------------

\newcommand{\Sh}{\ensuremath{\Pi_{\mathsf{Sh}}}}
\newcommand{\ShInt}{\ensuremath{\mathsf{ShInt}}}
\newcommand{\AngSh}{\ensuremath{\Pi_{\mathsf{aSh}}}}
\newcommand{\AngRec}{\ensuremath{\Pi_{\mathsf{aRec}}}}
\newcommand{\VASh}{\ensuremath{\Pi_{\mathsf{vaSh}}}}
\newcommand{\VARec}{\ensuremath{\Pi_{\mathsf{vaRec}}}}
\newcommand{\Rec}{\ensuremath{\Pi_{\mathsf{Rec}}}}
\newcommand{\FRec}{\ensuremath{\Pi_\mathsf{fRec}}}

\newcommand{\TripCheck}{\ensuremath{\Pi_\mathsf{prc}}}
\newcommand{\TripGen}{\ensuremath{\Pi_\mathsf{trip}}}
\newcommand{\MultiSenderOLE}{\ensuremath{\Pi_\mathsf{vm\mbox{-}ole}}}

\newcommand{\PiRand}{\ensuremath{\Pi_{\mathsf{rand}}}}
\newcommand{\PiCheckZero}{\ensuremath{\Pi_{\mathsf{CheckZero}}}}
\newcommand{\PiAdd}{\ensuremath{\Pi_{\mathsf{add}}}}
\newcommand{\PiMult}{\ensuremath{\Pi_{\mathsf{mult}}}}
\newcommand{\PiAddRing}{\ensuremath{\Pi^{\mathsf{sm,r}}_{\mathsf{add}}}}
\newcommand{\PiMultRing}{\ensuremath{\Pi^{\mathsf{sm,r}}_{\mathsf{mult}}}}
\newcommand{\PiMultRingComp}{\ensuremath{\Pi^{\mathsf{cm,r}}_{\mathsf{mult}}}}
\newcommand{\PiMultInt}{\ensuremath{\Pi_{\mathsf{Mult}}^{\mathsf{Int}}  }}
\newcommand{\PiZeroGen}{\ensuremath{\Pi_{\mathsf{ZeroGen}}}}
\newcommand{\PiConflict}{\ensuremath{\Pi_{\conflict}}}
%--------------------------------------------------------------
%ThreePC Functionalities
%--------------------------------------------------------------

\newcommand{\FSETUP}{\ensuremath{\mathcal{F}_{\mathsf{setup}}}}
\newcommand{\FTHREEMPC}{\ensuremath{\mathcal{F}_{\mathsf{3pc}}}}
\newcommand{\FTHREEMPCABORT}{\ensuremath{\mathcal{F}_{\mathsf{3pc}}^{\mathsf{Abort}}}}
\newcommand{\FTHREEMPCFAIR}{\ensuremath{\mathcal{F}_{\mathsf{3pc}}^{\mathsf{Fair}}}}
\newcommand{\FTRIPLES}{\ensuremath{\mathcal{F}_{\mathsf{trip}}}}
\newcommand{\FMULT}{\ensuremath{\mathcal{F}_{\mathsf{Mult}}}}
\newcommand{\FRAND}{\ensuremath{\mathcal{F}_{\mathsf{Rand}}}}
\newcommand{\FCOIN}{\ensuremath{\mathcal{F}_{\mathsf{Coin}}}}
\newcommand{\FINPUT}{\ensuremath{\mathcal{F}_{\mathsf{Input}}}}
\newcommand{\FCHECKZERO}{\ensuremath{\mathcal{F}_{\mathsf{CheckZero}}}}

%--------------------------------------------------------------
%ThreePC Protocols
%--------------------------------------------------------------

\newcommand{\PiThreeOnePerfectPassive}{\ensuremath{\Pi_{\mathsf{3pc}}^{\mathsf{pp}}}}
\newcommand{\PiThreeOneComputationalPassive}{\ensuremath{\Pi_{\mathsf{3pc}}^{\mathsf{cp}}}}
\newcommand{\PiThreeOneStatisticalActiveField}{\ensuremath{\Pi_{\mathsf{3pc}}^{\mathsf{sm,f}}}}
\newcommand{\PiThreeOneComputationalActiveField}{\ensuremath{\Pi_{\mathsf{3pc}}^{\mathsf{cm,f}}}}
\newcommand{\PiThreeOneStatisticalActiveRing}{\ensuremath{\Pi_{\mathsf{3pc}}^{\mathsf{sm,r}}}}
\newcommand{\PiThreeOneComputationalActiveRing}{\ensuremath{\Pi_{\mathsf{3pc}}^{\mathsf{cm,r}}}}

%--------------------------------------------------------------
%ThreePC Simulation
%--------------------------------------------------------------

\newcommand{\SPiThreeOnePerfectPassive}{\ensuremath{{\mathcal S}_{\mathsf{3pc}}^{\mathsf{pp}}}}
\newcommand{\SPiThreeOneStatisticalActiveRing}{\ensuremath{{\mathcal S}_{\mathsf{3pc}}^{\mathsf{sm}}}}


==> symbols/symbols_temp.tex <==
%--------------------------------------------------------------
%4PC Variables and Notations
%--------------------------------------------------------------
\newcommand{\addshare}[1]{\ensuremath{[#1]}}
\newcommand{\share}[1]{\ensuremath{\llbracket#1\rrbracket}}
\newcommand{\sha}[1]{\ensuremath{\rho_{#1}}}
\newcommand{\shb}[1]{\ensuremath{{m}_{#1}}}
\newcommand{\Share}[2]{\ensuremath{{\llbracket#1\rrbracket}_{P_{#2}}}}
\newcommand{\Sha}[2]{\ensuremath{[\alpha_{#1}]_{P_{#2}}}}
\newcommand{\Shb}[2]{\ensuremath{[\beta_{#1}]_{P_{#2}}}}
\newcommand{\AddSha}[2]{\ensuremath{[\alpha_{#1}]_{P_{#2}}}}
\newcommand{\AddShb}[2]{\ensuremath{[\beta_{#1}]_{P_{#2}}}}



%--------------------------------------------------------------
%4PC Protocols
%--------------------------------------------------------------

\newcommand{\SA}{\ensuremath{\mathsf{Abort4PC}}}
\newcommand{\Fair}{\ensuremath{\mathsf{fair4PC}}}
\newcommand{\Amultshare}{\ensuremath{\mathsf{A}}}
\newcommand{\Bmultshare}{\ensuremath{\mathsf{B}}}

%\newcommand{{\piaSh}}[1]{\ensuremath{\Pi^{#1}_{\Sh}}}
\newcommand{\shmask}[1]{\ensuremath{\sigma_{#1}}}


\newcommand{\shareB}[1]{\ensuremath{{\llbracket#1\rrbracket}^{\bf B}}}
\newcommand{\shareA}[1]{\ensuremath{{\llbracket#1\rrbracket}^{\bf A}}}


%--------------------------------------------------------------
% Special Conversions
%--------------------------------------------------------------

\newcommand{\BitExt}{\ensuremath{\mathsf{BitExt}}}
\newcommand{\piBitExt}{\ensuremath{\Pi_{\BitExt}}}
\newcommand{\PiBitExt}[2]{\ensuremath{\Pi_{\BitExt}({#1}, {#2})}}
%semi
\newcommand{\piBitExtS}{\ensuremath{\Pi^{\semi}_{\BitExt}}}
\newcommand{\PiBitExtS}[2]{\ensuremath{\Pi^{\semi}_{\BitExt}({#1}, {#2})}}
%malicious
\newcommand{\piBitExtM}{\ensuremath{\Pi^{\mal}_{\BitExt}}}
\newcommand{\PiBitExtM}[2]{\ensuremath{\Pi^{\mal}_{\BitExt}({#1}, {#2})}}

\newcommand{\SbiSemi}{\ensuremath{\Pi_{\mathsf{sbi}}^{\mathsf{semi}}}}
\newcommand{\GbiSemi}{\ensuremath{\Pi_{\mathsf{gbi}}^{\mathsf{semi}}}}
\newcommand{\SbiMal}{\ensuremath{\Pi_{\mathsf{sbi}}^{\mathsf{mal}}}}
\newcommand{\GbiMal}{\ensuremath{\Pi_{\mathsf{gbi}}^{\mathsf{mal}}}}

%\newcommand{\sqrA}[2]{[ #1 ]^{\bf{A}}_{#2}}


%--------------------------------------------------------------
% Building Blocks Protocols
%--------------------------------------------------------------
\newcommand{\piDP}{\ensuremath{\Pi_{\mathsf{dp}}}}
\newcommand{\PiDP}[3]{\ensuremath{\Pi_{\mathsf{dp}}({#1}, {#2},{#3})}}


\newcommand{\piSC}{\ensuremath{\Pi_{\mathsf{cmp}}}}
\newcommand{\PiSC}[2]{\ensuremath{\Pi_{\mathsf{cmp}}({#1}, {#2})}}

\newcommand{\piBT}{\ensuremath{\Pi_{\mathsf{btr}}}}
\newcommand{\PiBT}[2]{\ensuremath{\Pi_{\mathsf{btr}}({#1}, {#2})}}

\newcommand{\piBI}{\ensuremath{\Pi_{\mathsf{bin}}}}
\newcommand{\PiBI}[3]{\ensuremath{\Pi_{\mathsf{bin}}({#1}, {#2}, {#3})}}

\newcommand{\pidSh}{\ensuremath{\Pi_{\mathsf{dSh}}}}
\newcommand{\PidSh}[3]{\ensuremath{\Pi_{\mathsf{dSh}}({#1},{#2},{#3})}}

\newcommand{\piAMIN}{\ensuremath{\Pi_{\mathsf{ami}}}}
\newcommand{\PiAMIN}[2]{\ensuremath{\Pi_{\mathsf{ami}}({#1}, {#2})}}

\newcommand{\piAMX}{\ensuremath{\Pi_{\mathsf{amx}}}}
\newcommand{\PiAMX}[2]{\ensuremath{\Pi_{\mathsf{amx}}({#1}, {#2})}}

\newcommand{\piACT}{\ensuremath{\Pi_{\mathsf{act}}}}
\newcommand{\PiACT}[2]{\ensuremath{\Pi_{\mathsf{act}}({#1}, {#2})}}

%--------------------------------------------------------------
% Building Blocks Symbols
%--------------------------------------------------------------
\newcommand{\Aval}{\mathsf{a}}
\newcommand{\Bval}{\mathsf{b}}
